On Derandomizing Local Distributed Algorithms

The gap between the known randomized and deterministic local distributed algorithms underlies arguably the most fundamental and central open question in distributed graph algorithms. In this paper, we develop a generic and clean recipe for derandomizing LOCAL algorithms. We also exhibit how this simple recipe leads to significant improvements on a number of problem. Two main results are: - An improved distributed hypergraph maximal matching algorithm, improving on Fischer, Ghaffari, and Kuhn [FOCS'17], and giving improved algorithms for edge-coloring, maximum matching approximation, and low out-degree edge orientation. The first gives an improved algorithm for Open Problem 11.4 of the book of Barenboim and Elkin, and the last gives the first positive resolution of their Open Problem 11.10. - An improved distributed algorithm for the Lov\'{a}sz Local Lemma, which gets closer to a conjecture of Chang and Pettie [FOCS'17], and moreover leads to improved distributed algorithms for problems such as defective coloring and $k$-SAT.

==> derandomization.tex <==
\section{Basic Derandomization of Local Algorithms}
\label{sec:basic-derand-local}

\fabian{For now, I'm just the definitions from \cite{ghaffari2017complexity}.}

In the following assume that we are given a distributed graph problem
$\calP$ and a randomized $r$-round Monte Carlo algorithm $\calA$ for
$\calP$. 

\begin{lemma}
  Assume that we are given a distributed graph problem $\calP$ such
  that solutions to $\calP$ are a distributed language in $\ld[d]$
  (i.e., solutions are locally checkable in $d$ rounds). Further
  assume that we are given a randomized $\loc[r]$-algorithm $\calA$
  that computes a solution to $\calP$ with probability more than
  $1-1/n$. When running $\calA$ on a graph $G=(V,E)$, for each
  $v\in V$ let $R_v$ be the private random bit string used by node
  $v$. Then, there is a deterministic $\seqloc[2r+2d]$-algorithm that
  assigns values to all $R_v$ such that when (deterministically)
  running $\calA$ with those values, it solves $\calP$.
\end{lemma}
\begin{proof}
  We show how to derandomize the algorithm $\calA$ by using the method
  of conditional expectations. Consider a randomized run of
  $\calA$. For each node $v\in V$, we define an indicator random
  variable $F_v$ which is $F_v=1$ if and only if the output of the run
  of $\calA$ fails the local condition at node $v$. Note that since
  $\calA$ fails with probability less that $1/n$, it also holds for
  the individual local condition of each node $v$ that
  $\prob{F_v=1}<1/n$. Let us further define the random variable
  $F:=\sum_{v\in V} F_v$ such that $F>0$ if and only if $\calA$ fails
  to compute a solution for $\calP$. We note that by linearity of
  expectation, we have $\E[F] = \sum_{v\in V} \E[F_v] < 1$.

  We now show how to design a deterministic \seqloc-algorithm $\calA'$
  based on the randomized distributed algorithm $\calA$. We number the
  $n$ nodes in an arbitrary way from $v_1,\dots,v_n$ and assume that
  $\calA'$ processes the nodes in this order. When processing node
  $v_i$, $\calA'$ needs to fix the value of $R_{v_i}$. The goal of the
  algorithm is to pick values $r_i$ for all $i\in\set{1,\dots,n}$ such
  that for all $i\in\set{0,\dots,n}$, it holds that
  \begin{equation}\label{eq:condexpectation}
    \E\big[F \,\big|\, \set{R_{v_1}=r_1, \dots, R_{v_i}=r_i}\big] \leq \E[F]<1.
  \end{equation}
  After processing all $n$ nodes, all values $R_{v_i}$ are set to a
  fixed value and for $i=n$, the conditional expectation in
  \Cref{eq:condexpectation} is equal to the number of failed local
  conditions when running $\calA$ with these values for
  $R_{v_i}$. Because $\E[F]<1$, \Cref{eq:condexpectation} thus implies
  that $\E[F\,|\,R_{v_1}=r_1,\dots,R_{v_n}=r_n]=0$ and thus the
  algorithm succeeds in solving $\calP$. It remains to show how the
  values $r_i$ can be found such that \Cref{eq:condexpectation} is
  satisfied for all $i\in \set{0,\dots,n}$ and such that when
  processing node $v_i$, the \seqloc-algorithm $\calA'$ only needs to
  query the $(2r+2d)$-neighborhood of $v_I$. 


  If the values of $r_1,\dots,r_{i-1}$ are already given such that
  $\E[F\,|\,R_{v_1}=r_1,\dots,R_{v_{i-1}}=r_{i-1}]$,
  \Cref{eq:condexpectation} can clearly be satisfied by choosing $r_i$
  such that $\E[F\,|\,R_{v_1}=r_1,\dots,R_{v_i}=r_i]$ is
  minimized. Further note that for each node $v$, the value of $F_v$
  only depends on the outputs of $\calA$ of nodes within distance $d$
  from $v$ and $F_v$ therefore only depends on $R_u$ for nodes $u$
  within distance $r+d$ from $v$. Because the values of $R_u$ are
  mutually independent, for each node $v$ and all
  $S\subset V$, we therefore have
  \begin{equation}
    \label{eq:condindependence}
    \E\big[F_v\,\Bigg|\,\bigwedge_{u\in S} (R_u=r_u)\big] =
    \E\left[F_v\,\Bigg|\,\bigwedge_{u\in S \,:\, d_G(u,v)\leq r+d} (R_{u}=r_u)\right]
  \end{equation}
  We can therefore fix the value of $r_i$ as follows.
  \begin{eqnarray*}
    r_i 
    & = & \arg\min_{r}
          \E\big[F\,\big|\,R_{v_1}=r_1,\dots,R_{v_{i-1}}=r_{i-1},R_{v_i}=r]\\
    & = & \arg\min_{r} \sum_{v\in V}
          \E\big[F_v\,\big|\,R_{v_1}=r_1,\dots,R_{v_{i-1}}=r_{i-1},R_{v_i}=r]\\
    & = & \arg\min_r \sum_{v\,:\,d_G(v_i,v)\leq r+d} 
          \E\left[F_v\,\Bigg|\,R_i=r \land \bigwedge_{j< i \,:\,
          d_G(v,v_j)\leq r+d} (R_{v_j}=r_j)\right]
  \end{eqnarray*}
  The last equation follows because for $v$ at distance more than
  $r+d$ from $v_i$, by \Cref{eq:condindependence},
  $\E\big[F_v\,\big|\,R_{v_1}=r_1,\dots,R_{v_{i-1}}=r_{i-1},R_{v_i}=r]$
  does not depend on the value of $r$. Hence, when determining the
  value of $r_i$, $\calA'$ needs to evaluate
  conditional expectations of $F_v$ for all $v$ within distance at most
  $r+d$ from $v_i$. In order to do this, it is sufficient to read the
  current state of the $(2r+2d)$-neighborhood of $v_i$.
\end{proof}

\section{The Lov\'{a}sz Local Lemma}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "LOCALderandomization"
%%% End:

